Fast Linear Transformations in Python

Scientific computing requires handling large linear models, which are often composed of structured matrices. With increasing model size, dense representations quickly become infeasible to compute or store. Matrix-free implementations are suited to mitigate this problem but usually complicate research and development effort by months, when applied to practical research problems. Fastmat is a framework for handling large composed or structured matrices by offering an easy-to-use abstraction model. It allows expressing and using linear operators in a mathematically intuitive way, while maintaining a strong focus on efficient computation and memory storage. The implemented user interface allows for very readable code implementation with very close relationship to the actual mathematical notation of a given problem. Further it provides means for quickly testing new implementations and also allows for run-time execution path optimization. Summarizing, fastmat provides a flexible and extensible framework for handling matrix-free linear structured operators efficiently, while being intuitive and generating easy-to-reuse results.

==> tikz/muse_ground_truth_top_view.tex <==
\newcommand{\yPosOne}{18}
\newcommand{\yPosTwo}{13}
\newcommand{\circleRadiusOne}{1.5}
\newcommand{\circleRadiusTwo}{0.75}
\newcommand{\circleRadiusThree}{2.75}
\newcommand{\offsetOne}{20.7}
\newcommand{\offsetTwo}{65.7}
\newcommand{\offsetThree}{100.7}
\newcommand{\offsetFour}{160.7}
\newcommand{\offsetFive}{130.7}
\newcommand{\TenMMDeepHoles}{81.5}
\newcommand{\FifteenMMDeepHoles}{76.5}
\newcommand{\TwentyMMDeepHoles}{71.5}
\newcommand{\FiveMMDeepHoles}{86.5}
\newcommand{\linestyleGT}{densely dotted}
\newcommand{\linestyleFBHWalls}{dashed}

% Four holes on the left
\draw (axis cs: \offsetOne, \yPosOne) circle(\circleRadiusOne);
\draw (axis cs: \offsetOne+6, \yPosOne) circle(\circleRadiusOne);
\draw (axis cs: \offsetOne+20, \yPosOne) circle(\circleRadiusOne);
\draw (axis cs: \offsetOne+28, \yPosOne) circle(\circleRadiusOne);

% Three large holes diagonally placed
\draw (axis cs: \offsetTwo, \yPosTwo) circle(\circleRadiusOne);
\draw (axis cs: \offsetTwo+5, \yPosTwo+5) circle(\circleRadiusOne);
\draw (axis cs: \offsetTwo+10, \yPosTwo+10) circle(\circleRadiusOne);

% Three small holes diagonally placed
\draw (axis cs: \offsetThree, \yPosTwo) circle(\circleRadiusTwo);
\draw (axis cs: \offsetThree+5, \yPosTwo+5) circle(\circleRadiusTwo);
\draw (axis cs: \offsetThree+10, \yPosTwo+10) circle(\circleRadiusTwo);

% Three big holes second from right
\draw (axis cs: \offsetFive, \yPosOne) circle(\circleRadiusThree);
\draw (axis cs: \offsetFive+10, \yPosOne) circle(\circleRadiusThree);
\draw (axis cs: \offsetFive+20, \yPosOne) circle(\circleRadiusThree);

% Two small holes at the end
\draw (axis cs: \offsetFour, \yPosOne-0.25) circle(\circleRadiusTwo);
\draw (axis cs: \offsetFour+5.25, \yPosOne-0.25) circle(\circleRadiusTwo);
